Minimum Symbol Error Probability Low-Resolution Precoding for MU-MIMO Systems With PSK Modulation

We propose an optimal low-resolution precoding technique that minimizes the symbol error probability of the users. Unlike existing approaches that rely on QPSK modulation, for the derivation of the minimum symbol error probability objective function the current approach allows for any PSK modulation order. Moreover, the proposed method solves the corresponding discrete optimization problem optimally via a sophisticated branch-and-bound method. Moreover, we propose different approaches based on the greedy search method to compute practical solutions. Numerical simulations confirm the superiority of the proposed minimum symbol error probability criteria in terms of symbol error rate when compared with the established MMDDT and MMSE approaches.

==> Numerical_results/Figures/Complexity_Analysis.tex <==
    % This file was created by matlab2tikz v0.4.7 running on MATLAB 8.3.
% Copyright (c) 2008--2014, Nico Schlömer <nico.schloemer@gmail.com>
% All rights reserved.
% Minimal pgfplots version: 1.3
% 
% The latest updates can be retrieved from
%   http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz
% where you can also make suggestions and rate matlab2tikz.
% 
%
% defining custom colors
\usetikzlibrary{positioning,calc}

\definecolor{mycolor1}{rgb}{0.00000,1.00000,1.00000}%
\definecolor{mycolor2}{rgb}{1.00000,0.00000,1.00000}%
%

\pgfplotsset{every axis label/.append style={font=\footnotesize},
every tick label/.append style={font=\footnotesize}
}

\begin{tikzpicture}[font=\footnotesize] 

\begin{axis}[%
name=A ,
ymode=log,
width  = 0.4\columnwidth,%5.63489583333333in,
%width  = 0.4\columnwidth,%5.63489583333333in,
%height = 0.3\columnwidth,%4.16838541666667in,
height = 0.4\columnwidth,%4.16838541666667in,
scale only axis,
xmin  = -10,
xmax  = 20,
xlabel= {$\text{SNR}$},
xmajorgrids,
ymin=3,
ymax=600,
ylabel={$B$ },
ymajorgrids,
legend entries={MMSE \cite{MMSE_bb},
				MMDDT \cite{Landau2017},
                QMSEP Full-GS,
                UBMSEP Full-GS,
                QMSEP Partial-GS,
                UBMSEP Partial-GS,
                QMSEP UQ,
                UBMSEP UQ,
                },
%ytick={0, 0.5 , 1, 1.5, 2, 2.5 ,3,  3.1698  ,  4},
legend columns=2,
legend style={at={(0.13,0.234)},anchor=north west,draw=black,fill=white,legend cell align=left,font=\tiny}
]

\addlegendimage{color=blue,fill=gray!20,mark=pentagon}
\addlegendimage{color=red,fill=gray!20,mark=square}
\addlegendimage{color=dark_green,fill=gray!20,mark=o}
\addlegendimage{color=purple,fill=gray!20,mark=o}
\addlegendimage{color=dark_green,fill=gray!20,mark=diamond}
\addlegendimage{color=purple,fill=gray!20,mark=diamond}
\addlegendimage{color=dark_green,fill=gray!20,mark=asterisk}
\addlegendimage{color=purple,fill=gray!20,mark=asterisk}
%\addlegendimage{color=purple,dashed,fill=gray!20,mark=asterisk}

%PoPQ
%\addplot+[smooth,color=green,solid, every mark/.append style={solid, fill=gray!20},mark=square,
%y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
%  table[row sep=crcr]{%
%   0  0.013200856250000\\
%   1  0.012471784615385\\
%   2  0.011701737019231\\
%   3  0.010904155769231\\
%   4  0.010084902884615\\
%   5  0.009252383173077\\
%   6  0.008428209615385\\
%   7  0.007620877884615\\
%   8  0.006853329807692\\
%   9  0.006140354807692\\
%   10 0.005483773557692\\
%   11 0.004902665384615\\
%   12 0.004395031730769\\
%   13 0.003964064423077\\
%   14 0.003599219711538\\
%   15 0.003298030769231\\
%   16 0.003057620673077\\
%   17 0.002862022115385\\
%   18 0.002710360576923\\
%   19 0.002588457211538\\
%   20 0.002494077884615\\
%   21 0.002421959134615\\
%   22 0.002364371634615\\
%   23 0.002320342788462\\
%   24 0.002284522115385\\
%   25 0.002255893750000\\
%};



%% max min bb - alpha x 4 
\addplot+[smooth,color=red,solid, every mark/.append style={solid, fill=blue!20},mark=square,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      523.092500000000        \\
   -7.5000      523.092500000000        \\
   -5.0000      523.092500000000        \\
   -2.5000      523.092500000000        \\
         0      523.092500000000        \\
    2.5000      523.092500000000        \\
    5.0000      523.092500000000        \\
    7.5000      523.092500000000        \\
   10.0000      523.092500000000        \\
   12.5000      523.092500000000        \\
   15.0000      523.092500000000        \\
   17.5000      523.092500000000        \\
   20.0000      523.092500000000        \\
};


%mmmse - alpha x 4 
\addplot+[smooth,color=blue,solid, every mark/.append style={solid, fill=cyan!20},mark=pentagon,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      14.9450000000000        \\
   -7.5000      23.5250000000000        \\
   -5.0000      34.6700000000000        \\
   -2.5000      45.5300000000000        \\
         0      60.0475000000000        \\
    2.5000      81.4900000000000        \\
    5.0000      118.737500000000        \\
    7.5000      182.877500000000        \\
   10.0000      302.235000000000        \\
   12.5000      519.857500000000        \\
   15.0000      926.047500000000        \\
   17.5000      1655.81750000000        \\
   20.0000      2902.16000000000        \\
};


%qmsep uq  
\addplot+[smooth,color=dark_green,solid, every mark/.append style={solid, fill=cyan!20},mark=asterisk,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      4.56187500000000        \\
   -7.5000      10.4800000000000        \\
   -5.0000      21.8981250000000        \\
   -2.5000      36.2462500000000        \\
         0      54.5781250000000        \\
    2.5000      76.3806250000000        \\
    5.0000      107.310000000000        \\
    7.5000      153.507500000000        \\
   10.0000      209.882500000000        \\
   12.5000      221.207500000000        \\
   15.0000      128.573125000000        \\
   17.5000      35.7387500000000        \\
   20.0000      13.4525000000000        \\
};

%qmsep pgs 
\addplot+[smooth,color=dark_green,solid, every mark/.append style={solid, fill=cyan!20},mark=diamond,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      4.33187500000000        \\
   -7.5000      10.1025000000000        \\
   -5.0000      21.5106250000000        \\
   -2.5000      35.6662500000000        \\
         0      53.3631250000000        \\
    2.5000      73.9631250000000        \\
    5.0000      103.687500000000        \\
    7.5000      146.725000000000        \\
   10.0000      198.127500000000        \\
   12.5000      191.695000000000        \\
   15.0000      83.6106250000000        \\
   17.5000      14.3762500000000        \\
   20.0000      5.15250000000000        \\
};  

%qmsep fgs 
\addplot+[smooth,color=dark_green,solid, every mark/.append style={solid, fill=cyan!20},mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      30.5018750000000       \\
   -7.5000      36.2350000000000       \\
   -5.0000      42.9006250000000       \\
   -2.5000      51.1437500000000       \\
         0      63.0906250000000       \\
    2.5000      79.4531250000000       \\
    5.0000      105.130000000000       \\
    7.5000      145.850000000000       \\
   10.0000      193.020000000000       \\
   12.5000      184.445000000000       \\
   15.0000      77.9456250000000       \\
   17.5000      14.1662500000000       \\
   20.0000      5.38500000000000       \\
};

%ubmsep uq 
\addplot+[smooth,color=purple,solid, every mark/.append style={solid, fill=cyan!20},mark=asterisk,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      42.9718750000000    \\
   -7.5000      43.6737500000000    \\
   -5.0000      43.9237500000000    \\
   -2.5000      52.3100000000000    \\
         0      64.6468750000000    \\
    2.5000      82.7343750000000    \\
    5.0000      111.238125000000    \\
    7.5000      156.101250000000    \\
   10.0000      209.245000000000    \\
   12.5000      211.121875000000    \\
   15.0000      116.064375000000    \\
   17.5000      33.1331250000000    \\
   20.0000      9.77375000000000    \\
};

%ubmsep pgs
\addplot+[smooth,color=purple,solid, every mark/.append style={solid, fill=cyan!20},mark=diamond,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      37.6125000000000        \\
   -7.5000      40.9206250000000        \\
   -5.0000      46.5156250000000        \\
   -2.5000      55.3012500000000        \\
         0      66.4668750000000        \\
    2.5000      82.4581250000000        \\
    5.0000      108.116875000000        \\
    7.5000      148.787500000000        \\
   10.0000      196.265625000000        \\
   12.5000      180.326250000000        \\
   15.0000      73.7062500000000        \\
   17.5000      13.5168750000000        \\
   20.0000      5.21937500000000        \\
};

%ubmsep fgs
\addplot+[smooth,color=purple,solid, every mark/.append style={solid, fill=cyan!20},mark=o,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
  -10.0000      42.6331250000000        \\
   -7.5000      43.2756250000000        \\
   -5.0000      43.4881250000000        \\
   -2.5000      51.7643750000000        \\
         0      63.3581250000000        \\
    2.5000      79.6718750000000        \\
    5.0000      104.721875000000        \\
    7.5000      145.425000000000        \\
   10.0000      191.592500000000        \\
   12.5000      175.740625000000        \\
   15.0000      73.4693750000000        \\
   17.5000      13.4500000000000        \\
   20.0000      4.08625000000000        \\
};







\end{axis}





\begin{axis}[%
name=SumRate,
at={($(A.east)+(40,0em)$)},
                anchor= west,
name=B ,
ymode=log,
width  = 0.4\columnwidth,%5.63489583333333in,
%width  = 0.4\columnwidth,%5.63489583333333in,
%height = 0.3\columnwidth,%4.16838541666667in,
height = 0.4\columnwidth,%4.16838541666667in,
scale only axis,
xmin  = 3,
xmax  = 20,
xlabel= {$M$},
xmajorgrids,
ymin=3,
ymax=1000,
ylabel={$B$ },
ymajorgrids,
%legend entries={Ex. Search,
%				MMSE-B\&B,
%				MMDDT-B\&B    \cite{Landau2017}
%                %$M=14$,
%                %$M=16$,
%                },
%%ytick={0, 0.5 , 1, 1.5, 2, 2.5 ,3,  3.1698  ,  4},
%legend style={at={(0,1)},anchor=north west,draw=black,fill=white,legend cell align=left,font=\tiny}
]

\addlegendimage{color=black,dashed,fill=gray!20,mark=asterisk}
\addlegendimage{color=blue,fill=gray!20,mark=pentagon}
%\addlegendimage{only marks,color=black,fill=green!20,mark=triangle}
%\addlegendimage{only marks,color=black,fill=red!20,mark=o}
\addlegendimage{color=red,fill=gray!20,mark=square}

%\addlegendimage{color=black,fill=gray!20,mark=asterisk}
%\addlegendimage{color=black,fill=gray!20,mark=triangle}
%\addlegendimage{only marks,color=black,fill=green!20,mark=triangle}
%\addlegendimage{only marks,color=black,fill=red!20,mark=o}
%\addlegendimage{color=black,fill=gray!20,mark=square}

%FOR THE FIRST VALUE OF M

%Ehaustive Search
\addplot+[smooth,color=black,dashed, every mark/.append style={solid, fill=gray!20},mark=asterisk,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
3	64	\\
4	256	\\
5	1024	\\
6	4096	\\
7	16384	\\
8	65536	\\
9	262144	\\
10	1048576	\\
11	4194304	\\
12	16777216	\\
13	67108864	\\
14	268435456	\\
15	1073741824	\\
16	4294967296	\\
17	17179869184	\\
18	68719476736	\\
19	2.74878E+11	\\
20	1.09951E+12	\\
};


%1-bit Landau 2017
\addplot+[smooth,color=red,solid, every mark/.append style={solid, fill=cyan!20},mark=square,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
%\\\\\2	7.4625	\\
%\\\\\2	7.4625	\\
3	12.4675	\\
4	25.4545	\\
5	44.5475	\\
6	71.5485	\\
7	107.082	\\
8	153.87	\\
9	218.9895	\\
10	288.626	\\
11	405.48	\\
12	525.95	\\
13	709.69	\\
14	868.6	\\
15	1108.07	\\
16	1450.82	\\
17	1752.1	\\
18	2204.44	\\
19	2620.24	\\
20	3222.01	\\
21	3862.5305	\\
22	4657.18375	\\
23	5583.9215	\\
24	6560.86	\\
25	7.80E+03	\\
};


%mmse bb - alpha x 4
\addplot+[smooth,color=blue,solid, every mark/.append style={solid, fill=cyan!20},mark=pentagon,
y filter/.code={\pgfmathparse{\pgfmathresult-0}\pgfmathresult}]
  table[row sep=crcr]{%
%\\\\\2	7.4625	\\
3	6.0975	\\
4	10.6188	\\
5	15.5013	\\
6	19.8313	\\
7	26.3012	\\
8	31.2963	\\
9	37.5662	\\
10	43.7612	\\
11	52.195	\\
12	60.1325	\\
13	63.945	\\
14	72.6325	\\
15	80.6025	\\
16	90.8662	\\
17	100.1513	\\
18	108.1688	\\
19	118.9875	\\
20	131.1763	\\
};








%\node [draw,fill=white,font=\tiny,anchor= south  east] at (axis %cs: 20,7) {
%%\setlength{\tabcolsep}{0.5mm}
%%\renewcommand{\arraystretch}{.8}
%\begin{tabular}{l}
%\ref{P99}{$\alpha_x=4$}\\
%\ref{P88}{$\alpha_x=3$}\\
%\end{tabular}
%};






\end{axis}







\end{tikzpicture}%

==> Precoder/01_QoS_BnB.tex <==
\section{Reduced Complexity Branch-and-Bound under QoS}
\label{sec:qos_bnb}
Previous B\&B methods used indirect optimization criteria to minimize the SEP. However, when utilizing the MSEP criteria one can easily compute the SEP of a transmit vector $\boldsymbol{x}$. As such, the algorithm can also support the case where only a suboptimal solution that attains a SEP constraint is required.
Considering the case where a QoS constraint vector $\boldsymbol{\lambda} \in (0,1]^K $ is provided, the algorithm computes the SEP of each upper bound solution $\boldsymbol{x}_{\text{ub}|\boldsymbol{f}}$ and checks if it is smaller or equal to $\boldsymbol{\lambda}$, if so the algorithm returns $\boldsymbol{x}_{\text{ub}|\boldsymbol{f}}$.
In the QMSEP case, for a given $\boldsymbol{x}$, the SEP is computed as 
\begin{align}
\label{eq:er_prob_qmsep}
    \text{\textbf{P}}_\text{e}\pc{\hat{\boldsymbol{s}}|\boldsymbol{x}}=\boldsymbol{1}_K^T - \Phi\pc{\boldsymbol{S}_\text{r}\  \text{Re}\chav{\boldsymbol{Hx}}} \circ \Phi\pc{\boldsymbol{S}_\text{i}\ \text{Im}\chav{\boldsymbol{Hx}}},
\end{align}
where $\circ$ denotes elementwise multiplication. In the UBMSEP case, for a given $\boldsymbol{x}$, the SEP is computed as 
\begin{align}
\label{eq:prob_ubmsep}
    \text{\textbf{P}}_\text{e}\pc{\hat{\boldsymbol{s}}|\boldsymbol{x}}=    \text{Q}\pc{\text{Re}\chav{\boldsymbol{H}^\text{s} \boldsymbol{x}}-\text{Im}\chav{\boldsymbol{H}^\text{c}  \boldsymbol{x}}}+
    \text{Q}\pc{ \text{Re}\chav{\boldsymbol{H}^\text{s} \boldsymbol{x}}+\text{Im}\chav{\boldsymbol{H}^\text{c}  \boldsymbol{x}}}.
\end{align}
This method can significantly reduce the total number of evaluated branches in the B\&B algorithm. The steps of the MSEP B\&B algorithm under QoS are detailed in in Algorithm~\ref{alg:MSEP_QoS}. 

\input{Precoder/Algorithms/Alg_MSEP_QoS}


==> Precoder/Algorithms/Alg_MSEP_QoS.tex <==
\begin{algorithm}
\small
  \caption{Proposed MSEP QoS B\&B Precoding Algorithm}
	\label{alg:MSEP_QoS} 
  \begin{algorithmic}    %[1] %for numbers
  \State{\textbf{Inputs}: $\mathcal{M}(\cdot)$, MSEP criterion, $g(\boldsymbol{x})$, $\boldsymbol{\lambda}$ and $\text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{x})$ \hspace{1em} \textbf{Output}: $\boldsymbol{x}_\text{out}$ }
    \State{Solve the relaxed optimization problem corresponding to the MSEP criterion and get $\boldsymbol{x}_\text{r,lb}$}
    \State{Project $\boldsymbol{x}_\text{r,lb}$ to get the upper bound solution $\boldsymbol{x}_\text{ub}=\mathcal{M}(C(\boldsymbol{x}_\text{r,lb}))$ and compute $\text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{x}_\text{ub})$}
    \State{\textbf{If} $\boldsymbol{x}_\text{ub}==\boldsymbol{x}_\text{lb} \ \land \ \text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{x}_\text{ub})\leq \boldsymbol{\lambda}$ }
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=\boldsymbol{x}_\text{ub}$ }
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Define $\check{\boldsymbol{x}}=\boldsymbol{x}_\text{ub}$ and compute $\check{g}=g(\check{\boldsymbol{x}})$ }
    \State{Define the first level ($p=1$) of the tree by $\mathcal{G}_{p}:=\mathcal{X}_{\textrm{}}$}
	\For{$p=1:M-1$}
	\State{Partition  $\mathcal{G}_{p}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\PM{\mathcal{G}_{p}}}$ } 
	  \For{$i=1:\left| \mathcal{G}_{p} \right|$}
		\State{Conditioned on $\boldsymbol{f}_{\text{r},i}=R(\boldsymbol{f}_{i})$ solve the subproblem corresponding to the MSEP criterion to get $\boldsymbol{v}_{\text{r,lb}|f_{i}}$}
		\State{Construct $\boldsymbol{x}_{\text{lb,}i}=\pr{\boldsymbol{f}_{i}^T\ , \ C\pc{\boldsymbol{v}_{\text{r,lb}|f_{i}} }^T}$ and determine the lower bound $g_{\text{lb},i}=g(\boldsymbol{x}_{\text{lb,}i})$ }
		\State{Project $\boldsymbol{x}_{\text{lb,}i}$ to get the upper bound solution $\boldsymbol{x}_{\text{ub,}i}=\mathcal{M}(\boldsymbol{x}_{\text{lb,}i})$ and compute $\text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{x}_\text{ub,i})$}
		\State{\textbf{If} $\text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{x}_{\text{ub},i})\leq \boldsymbol{\lambda}$ }
        \vspace{-0.5em}
        \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=\boldsymbol{x}_{\text{ub},i}$ }
        \vspace{-0.5em}
        \State{\textbf{end if} }
		\State{With $\boldsymbol{x}_{\textrm{ub,i}}$ compute the upper bound $g_{\text{ub},i}=g(\boldsymbol{x}_{\text{ub,}i})$}
		\State{Update the best upper bound as $\check{g} =\min\left( \check{g}, g_{\text{ub},i}  \right)$ and update $\check{\boldsymbol{x}}$ accordingly} 
	\EndFor
	\State{Construct a reduced set by comparing conditioned  lower bounds with the global upper bound $\check{g}$}
	\State{$\mathcal{G}_{p}^{\prime}:=\left\{  \boldsymbol{x}_{\text{lb},i}\ \vert\  g_{\textrm{lb},i} < (1-\gamma) \ \check{g}       , i=1,\ldots,  \left|\mathcal{G}_{p}\right|  \right\} $}
	\State{Define the set for the next level in the tree: $\mathcal{G}_{p+1}:=\mathcal{G}_{p}^{\prime} \times \mathcal{X}_{\textrm{}}$}
	%\vspace{-0.5em}
	%\State{\textcolor{r}{\textbf{end if}}}
	\EndFor
	\State{Partition $\mathcal{G}_{M}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\left|\mathcal{G}_{M}\right|}$}
	\For {$i=1:\PM{\mathcal{G}_M}$}
	\State{Conditioned on $\boldsymbol{f}_{i}$ compute $g(\boldsymbol{f}_{i})$ and $\text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{f}_{i})$}
	\State{\textbf{If}  $\text{\textbf{P}}_\text{e}(\hat{\boldsymbol{s}}|\boldsymbol{f}_{i})\leq \boldsymbol{\lambda}$ }
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return}
    $\boldsymbol{x}_\text{out}=\boldsymbol{f}_i$}
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Update $\check{g} =\min\left( \check{g}, g(\boldsymbol{f}_{i})  \right)$ and update $\check{\boldsymbol{x}}$ accordingly}
	\EndFor
	\State{The global solution is $\boldsymbol{x}_{\textrm{out}} =\check{\boldsymbol{x}}$}
\end{algorithmic}
\end{algorithm}

==> Precoder/Algorithms/Alg_QMSEP.tex <==
\begin{algorithm}
\small
  \caption{Proposed QMSEP B\&B Precoding Algorithm}
	\label{alg:QMSEP}
  \begin{algorithmic}    %[1] %for numbers
  \State{\textbf{Inputs}: $\mathcal{M}(\cdot)$, $\boldsymbol{H}$, $\boldsymbol{s}$ and $\sigma_w^2$ \hspace{1em} \textbf{Output}: $\boldsymbol{x}_\text{out}$ }
    \State{Solve the optimization problem described in \eqref{eq:qmsep_mapped_prob} and get $\boldsymbol{x}_\text{r,lb}$}
    \State{Project $\boldsymbol{x}_\text{lb}=R(\boldsymbol{x}_\text{r,lb})$ to get the upper bound solution $\boldsymbol{x}_\text{ub}=\mathcal{M}(\boldsymbol{x}_\text{lb})$ }
    \State{\textbf{If} $\boldsymbol{x}_\text{ub}==\boldsymbol{x}_\text{lb}$}
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=\boldsymbol{x}_\text{ub}$ }
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Define $\check{\boldsymbol{x}}=\boldsymbol{x}_\text{ub}$ and compute $\check{g}=g(\check{\boldsymbol{x}})$ using equation \eqref{eq:g_qmsep} }
    \State{Define the first level ($p=1$) of the tree by $\mathcal{G}_{p}:=\mathcal{X}_{\textrm{}}$}
	\For{$p=1:M-1$}
	\State{Partition  $\mathcal{G}_{p}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\PM{\mathcal{G}_{p}}}$ }  
	  \For{$i=1:\left| \mathcal{G}_{p} \right|$}
		\State{Conditioned on $\boldsymbol{f}_{\text{r},i}=R(\boldsymbol{f}_{i})$ solve \eqref{eq:qpsk_sub_prob} to get $\boldsymbol{v}_{\text{r,lb}|f_{i}}$}
		\State{Construct $\boldsymbol{x}_{\text{lb,}i}=\pr{\boldsymbol{f}_{i}^T\ , \ C\pc{\boldsymbol{v}_{\text{r,lb}|f_{i}} }^T}$ and determine the lower bound $g_{\text{lb},i}=g(\boldsymbol{x}_{\text{lb,}i})$ using \eqref{eq:g_qmsep} }
		\State{Compute the upper bound $\boldsymbol{x}_{\text{ub,}i}=\mathcal{M}(\boldsymbol{x}_{\text{lb,}i})$}
		\State{With $\boldsymbol{x}_{\textrm{ub,i}}$ compute the upper bound $g_{\text{ub},i}=g(\boldsymbol{x}_{\text{ub,}i})$ using \eqref{eq:g_qmsep} }
		\State{Update the best upper bound as $\check{g} =\min\left( \check{g}, g_{\text{ub},i}  \right)$ and update $\check{\boldsymbol{x}}$ accordingly} 
	\EndFor
	\State{Construct a reduced set by comparing conditioned  lower bounds with the global upper bound $\check{g}$}
	\State{$\mathcal{G}_{p}^{\prime}:=\left\{  \boldsymbol{x}_{\text{lb},i}\ \vert\  g_{\textrm{lb},i} < (1-\gamma) \ \check{g}       , i=1,\ldots,  \left|\mathcal{G}_{p}\right|  \right\} $}
	\State{Define the set for the next level in the tree: $\mathcal{G}_{p+1}:=\mathcal{G}_{p}^{\prime} \times \mathcal{X}_{\textrm{}}$}
	%\vspace{-0.5em}
	%\State{\textcolor{r}{\textbf{end if}}}
	\EndFor
	\vspace{1mm}
	\State{Search method for the last layer $p=M$,}
	\vspace{1mm}
	\State{The global solution is $\boldsymbol{x}_{\textrm{out}} = \mathrm{arg} \hspace{-6mm}\displaystyle \min_{\boldsymbol{x} \in \chav{\mathcal{G}_M \cup \chav{\check{\boldsymbol{x}}}}  } g (\boldsymbol{x})$ }
\end{algorithmic}
\end{algorithm}

==> Precoder/Algorithms/Alg_UBMSEP.tex <==
\begin{algorithm}
\small
  \caption{Proposed UB-MSEP B\&B Precoding Algorithm}
	\label{alg:UB-MSEP}
  \begin{algorithmic}    %[1] %for numbers
  \State{\textbf{Inputs}: $\mathcal{M}(\cdot)$, $\boldsymbol{H}$, $\boldsymbol{s}$, $\theta$ and $\sigma_w^2$ \hspace{1em} \textbf{Output}: $\boldsymbol{x}_\text{out}$ }
    \State{Solve the optimization problem described in \eqref{eq:ub_msep_problem} and get $\boldsymbol{x}_\text{r,lb}$}
    \State{Project $\boldsymbol{x}_\text{lb}=R(\boldsymbol{x}_\text{r,lb})$ to get the upper bound solution $\boldsymbol{x}_\text{ub}=\mathcal{M}(\boldsymbol{x}_\text{lb})$ }
    \State{\textbf{If} $\boldsymbol{x}_\text{ub}==\boldsymbol{x}_\text{lb}$}
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=\boldsymbol{x}_\text{ub}$ }
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Define $\check{\boldsymbol{x}}=\boldsymbol{x}_\text{ub}$ and compute $\check{g}=g(\check{\boldsymbol{x}})$ using equation \eqref{eq:g_ubmsep} }
    \State{Define the first level ($p=1$) of the tree by $\mathcal{G}_{p}:=\mathcal{X}_{\textrm{}}$}
	\For{$p=1:M-1$}
	\State{Partition  $\mathcal{G}_{p}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\PM{\mathcal{G}_{p}}}$ }  
	  \For{$i=1:\left| \mathcal{G}_{p} \right|$}
		\State{Conditioned on $\boldsymbol{f}_{\text{r},i}=R(\boldsymbol{f}_{i})$ solve \eqref{eq:PSK_sub_problem_relaxed} to get $\boldsymbol{v}_{\text{r,lb}|f_{i}}$}
		\State{Construct $\boldsymbol{x}_{\text{lb,}i}=\pr{\boldsymbol{f}_{i}^T\ , \ C\pc{\boldsymbol{v}_{\text{r,lb}|f_{i}} }^T}$ and determine the lower bound $g_{\text{lb},i}=g(\boldsymbol{x}_{\text{lb,}i})$ using \eqref{eq:g_ubmsep} }
		\State{Compute the upper bound $\boldsymbol{x}_{\text{ub,}i}=\mathcal{M}(\boldsymbol{x}_{\text{lb,}i})$}
		\State{With $\boldsymbol{x}_{\textrm{ub,i}}$ compute the upper bound $g_{\text{ub},i}=g(\boldsymbol{x}_{\text{ub,}i})$ using \eqref{eq:g_ubmsep} }
		\State{Update the best upper bound as $\check{g} =\min\left( \check{g}, g_{\text{ub},i}  \right)$ and update $\check{\boldsymbol{x}}$ accordingly} 
	\EndFor
	\State{Construct a reduced set by comparing conditioned  lower bounds with the global upper bound $\check{g}$}
	\State{$\mathcal{G}_{p}^{\prime}:=\left\{  \boldsymbol{x}_{\text{lb},i}\ \vert\  g_{\textrm{lb},i} < (1-\gamma) \ \check{g}       , i=1,\ldots,  \left|\mathcal{G}_{p}\right|  \right\} $}
	\State{Define the set for the next level in the tree: $\mathcal{G}_{p+1}:=\mathcal{G}_{p}^{\prime} \times \mathcal{X}_{\textrm{}}$}
	%\vspace{-0.5em}
	%\State{\textcolor{r}{\textbf{end if}}}
	\EndFor
	\vspace{1mm}
	\State{Search method for the last layer $p=M$,}
	\vspace{1mm}
	\State{The global solution is $\boldsymbol{x}_{\textrm{out}} = \mathrm{arg} \hspace{-6mm}\displaystyle \min_{\boldsymbol{x} \in \chav{\mathcal{G}_M \cup \chav{\check{\boldsymbol{x}}}}  } g (\boldsymbol{x})$ }
\end{algorithmic}
\end{algorithm}

==> Precoder/Algorithms/Alg_qmsep_qos.tex <==
\begin{algorithm}
\small
  \caption{Proposed QMSEP QoS B\&B Precoding Algorithm}
	\label{alg:QMSEP_QoS}
  \begin{algorithmic}    %[1] %for numbers
  \State{\textbf{Inputs}: $\boldsymbol{H}$, $\boldsymbol{s}$, $\boldsymbol{\lambda}$ and $\sigma_w^2$ \hspace{1em} \textbf{Output}: $\boldsymbol{x}_\text{out}$ }
    \State{Solve the optimization problem described in \eqref{eq:qmsep_mapped_prob} and get $\boldsymbol{x}_\text{r,lb}$}
    \State{Project $\boldsymbol{x}_\text{r,lb}$, using Algorithm \ref{alg:QMSEP_GS}, to get the upper bound solution $\boldsymbol{x}_\text{r,ub}=\mathcal{M}(\boldsymbol{x}_\text{r,lb})$ }
    \State{Compute $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_\text{r,ub})$} with \eqref{eq:er_prob_qmsep}
    \State{\textbf{If} $\boldsymbol{x}_\text{r,ub}==\boldsymbol{x}_\text{r,lb} \ \land \ \text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_\text{r,ub})\leq \boldsymbol{\lambda}$ }
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=C(\boldsymbol{x}_\text{r,ub})$ }
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Define $\check{\boldsymbol{x}}_\text{r}=\boldsymbol{x}_\text{r,ub}$ and compute $\check{g}=g(\check{\boldsymbol{x}}_\text{r})$ using equation \eqref{eq:g_qmsep} }
    \State{Define the first level ($p=1$) of the tree by $\mathcal{G}_{p}:=\mathcal{X}_{\textrm{}}$}
	\For{$p=1:M-1$}
	\State{Partition  $\mathcal{G}_{p}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\PM{\mathcal{G}_{p}}}$ }  
	  \For{$i=1:\left| \mathcal{G}_{p} \right|$}
		\State{Conditioned on $\boldsymbol{f}_{\text{r},i}=R(\boldsymbol{f}_{i})$ solve \eqref{eq:qpsk_sub_prob} to get $\boldsymbol{v}_{\text{r,lb}|f_{i}}$}
		\State{Construct $\boldsymbol{x}_{\text{r,lb,}i}=\pr{\boldsymbol{f}_{\text{r},i}^T\ , \ \boldsymbol{v}^T_{\text{r}|f_{i}} }$ and determine the lower bound $g_{\text{lb},i}=g(\boldsymbol{x}_{\text{r,lb,}i})$ using \eqref{eq:g_qmsep} }
		\State{Compute the upper bound $\boldsymbol{x}_{\text{r,ub,}i}=\mathcal{M}(\boldsymbol{x}_{\text{r,lb,}i})$ using Algorithm \ref{alg:QMSEP_GS} }
		\State{Using \eqref{eq:er_prob_qmsep} compute the probabilities $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_\text{r,ub,i})$}
		\State{\textbf{If} $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_{\text{r,ub},i})\leq \boldsymbol{\lambda}$ }
        \vspace{-0.5em}
        \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=C(\boldsymbol{x}_{\text{r,ub},i})$ }
        \vspace{-0.5em}
        \State{\textbf{end if} }
		\State{With $\boldsymbol{x}_{\textrm{r,ub,i}}$ compute the upper bound $g_{\text{ub},i}=g(\boldsymbol{x}_{\text{r,ub,}i})$ using \eqref{eq:g_qmsep} }
		\State{Update the best upper bound as $\check{g} =\min\left( \check{g}, g_{\text{ub},i}  \right)$ and update $\check{\boldsymbol{x}}_\text{r}$ accordingly} 
	\EndFor
	\State{Construct a reduced set by comparing conditioned  lower bounds with the global upper bound $\check{g}$}
	\State{$\mathcal{G}_{p}^{\prime}:=\left\{  \boldsymbol{x}_{\text{r,lb},i}\ \vert\  g_{\textrm{lb},i} < (1-\gamma) \ \check{g}       , i=1,\ldots,  \left|\mathcal{G}_{p}\right|  \right\} $}
	\State{Define the set for the next level in the tree: $\mathcal{G}_{p+1}:=\mathcal{G}_{p}^{\prime} \times \mathcal{X}_{\textrm{}}$}
	%\vspace{-0.5em}
	%\State{\textcolor{r}{\textbf{end if}}}
	\EndFor
	\State{Partition $\mathcal{G}_{M}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\left|\mathcal{G}_{M}\right|}$}
	\For {$i=1:\PM{\mathcal{G}_M}$}
	\State{Conditioned on $\boldsymbol{f}_{\text{r},i}= R(\boldsymbol{f}_i)$} compute $g(\boldsymbol{f}_{\text{r},i})$ and $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{f}_{\text{r},i})$
	\State{\textbf{If}  $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{f}_{\text{r},i})\leq \boldsymbol{\lambda}$ }
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return}
    $\boldsymbol{x}_\text{out}=C(\boldsymbol{f}_i)$}
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Update $\check{g} =\min\left( \check{g}, g(\boldsymbol{f}_{\text{r},i})  \right)$ and update $\check{\boldsymbol{x}}_\text{r}$ accordingly}
	\EndFor
	\State{The global solution is $\boldsymbol{x}_{\textrm{out}} =C(\check{\boldsymbol{x}}_\text{r})$}
\end{algorithmic}
\end{algorithm}

==> Precoder/Algorithms/Alg_ubmsep_qos.tex <==
\begin{algorithm}
\small
  \caption{Proposed UB-MSEP QoS B\&B Precoding Algorithm}
	\label{alg:UBMSEP_QoS} 
  \begin{algorithmic}    %[1] %for numbers
  \State{\textbf{Inputs}: $\boldsymbol{H}$, $\boldsymbol{s}$, $\boldsymbol{\lambda}$, $\theta$ and $\sigma_w^2$ \hspace{1em} \textbf{Output}: $\boldsymbol{x}_\text{out}$ }
    \State{Solve the optimization problem described in \eqref{eq:ub_msep_problem} and get $\boldsymbol{x}_\text{r,lb}$}
    \State{Project $\boldsymbol{x}_\text{r,lb}$, using Algorithm \ref{alg:UBMSEP_GS}, to get the upper bound solution $\boldsymbol{x}_\text{r,ub}=\mathcal{M}(\boldsymbol{x}_\text{r,lb})$ }
    \State{Compute $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_\text{r,ub})$} with \eqref{eq:prob_ubmsep}
    \State{\textbf{If} $\boldsymbol{x}_\text{r,ub}==\boldsymbol{x}_\text{r,lb} \ \land \ \text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_\text{r,ub})\leq \boldsymbol{\lambda}$ }
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=C(\boldsymbol{x}_\text{r,ub})$ }
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Define $\check{\boldsymbol{x}}_\text{r}=\boldsymbol{x}_\text{r,ub}$ and compute $\check{g}=g(\check{\boldsymbol{x}}_\text{r})$ using equation \eqref{eq:g_ubmsep} }
    \State{Define the first level ($p=1$) of the tree by $\mathcal{G}_{p}:=\mathcal{X}_{\textrm{}}$}
	\For{$p=1:M-1$}
	\State{Partition  $\mathcal{G}_{p}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\PM{\mathcal{G}_{p}}}$ }  
	  \For{$i=1:\left| \mathcal{G}_{p} \right|$}
		\State{Conditioned on $\boldsymbol{f}_{\text{r},i}=R(\boldsymbol{f}_{i})$ solve \eqref{eq:PSK_sub_problem_relaxed} to get $\boldsymbol{v}_{\text{r,lb}|f_{i}}$}
		\State{Construct $\boldsymbol{x}_{\text{r,lb,}i}=\pr{\boldsymbol{f}_{\text{r},i}^T\ , \ \boldsymbol{v}^T_{\text{r}|f_{i}} }$ and determine the lower bound $g_{\text{lb},i}=g(\boldsymbol{x}_{\text{r,lb,}i})$ using \eqref{eq:g_ubmsep} }
		\State{Compute the upper bound $\boldsymbol{x}_{\text{r,ub,}i}=\mathcal{M}(\boldsymbol{x}_{\text{r,lb,}i})$ using Algorithm \ref{alg:UBMSEP_GS} }
		\State{Using \eqref{eq:prob_ubmsep} compute the probabilities $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_\text{r,ub,i})$}
		\State{\textbf{If} $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{x}_{\text{r,ub},i})\leq \boldsymbol{\lambda}$ }
        \vspace{-0.5em}
        \State{\hspace{1em} \textbf{return} $\boldsymbol{x}_\text{out}=C(\boldsymbol{x}_{\text{r,ub},i})$ }
        \vspace{-0.5em}
        \State{\textbf{end if} }
		\State{With $\boldsymbol{x}_{\textrm{r,ub,i}}$ compute the upper bound $g_{\text{ub},i}=g(\boldsymbol{x}_{\text{r,ub,}i})$ using \eqref{eq:g_ubmsep} }
		\State{Update the best upper bound as $\check{g} =\min\left( \check{g}, g_{\text{ub},i}  \right)$ and update $\check{\boldsymbol{x}}_\text{r}$ accordingly} 
	\EndFor
	\State{Construct a reduced set by comparing conditioned  lower bounds with the global upper bound $\check{g}$}
	\State{$\mathcal{G}_{p}^{\prime}:=\left\{  \boldsymbol{x}_{\text{r,lb},i}\ \vert\  g_{\textrm{lb},i} < (1-\gamma) \ \check{g}       , i=1,\ldots,  \left|\mathcal{G}_{p}\right|  \right\} $}
	\State{Define the set for the next level in the tree: $\mathcal{G}_{p+1}:=\mathcal{G}_{p}^{\prime} \times \mathcal{X}_{\textrm{}}$}
	%\vspace{-0.5em}
	%\State{\textcolor{r}{\textbf{end if}}}
	\EndFor
	\State{Partition $\mathcal{G}_{M}$ in $\boldsymbol{f}_{1},\ldots,\boldsymbol{f}_{\left|\mathcal{G}_{M}\right|}$}
	\For {$i=1:\PM{\mathcal{G}_M}$}
	\State{Conditioned on $\boldsymbol{f}_{\text{r},i}= R(\boldsymbol{f}_i)$} compute $g(\boldsymbol{f}_{\text{r},i})$ and $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{f}_{\text{r},i})$
	\State{\textbf{If}  $\text{\textbf{P}}_\text{e}(\boldsymbol{s}|\boldsymbol{f}_{\text{r},i})\leq \boldsymbol{\lambda}$ }
    \vspace{-0.5em}
    \State{\hspace{1em} \textbf{return}
    $\boldsymbol{x}_\text{out}=C(\boldsymbol{f}_i)$}
    \vspace{-0.5em}
    \State{\textbf{end if} }
    \State{Update $\check{g} =\min\left( \check{g}, g(\boldsymbol{f}_{\text{r},i})  \right)$ and update $\check{\boldsymbol{x}}_\text{r}$ accordingly}
	\EndFor
	\State{The global solution is $\boldsymbol{x}_{\textrm{out}} =C(\check{\boldsymbol{x}}_\text{r})$}
\end{algorithmic}
\end{algorithm}
